ELMGS: Enhancing memory and computation scaLability through coMpression for 3D Gaussian Splatting

3D models have recently been popularized by the potentiality of end-to-end training offered first by Neural Radiance Fields and most recently by 3D Gaussian Splatting models. The latter has the big advantage of naturally providing fast training convergence and high editability. However, as the research around these is still in its infancy, there is still a gap in the literature regarding the model's scalability. In this work, we propose an approach enabling both memory and computation scalability of such models. More specifically, we propose an iterative pruning strategy that removes redundant information encoded in the model. We also enhance compressibility for the model by including in the optimization strategy a differentiable quantization and entropy coding estimator. Our results on popular benchmarks showcase the effectiveness of the proposed approach and open the road to the broad deployability of such a solution even on resource-constrained devices.

==> display_figures/Supplementary_Figures/memory_consumption.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/Supplementary_Figures/Memory_Consumption.pdf}
    \caption{Memory savings while training using Gradient and Opacity based Pruning (GAP) on Tanks\&Temples dataset.}
    \label{sup-fig:memory_savings}
    \vspace{-10pt}
\end{figure*}

==> display_figures/fps.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/FPS_TandT.pdf}
    \caption{Tradeoff between performance and size in terms of FPS on Tanks\&Temples dataset.}
    \label{fig:fps}
\end{figure}

==> display_figures/opacity_comp.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/b_p_opacity(1).pdf}
    \caption{Opacity distribution before and after GAP for the \texttt{garden} scene}
    \label{fig:opacity-comp}
\end{figure}

==> display_figures/ours_medium.tex <==
\begin{figure*}
\caption{Comparison of ground truth images from the test set between ours-medium compressed representation and 3DGS-30k}
\vspace{-0.2cm}
\includegraphics[width=\linewidth]{figures/ours_medium.pdf}
    \centering

    \label{fig:ours-medium}
    
\end{figure*}

==> display_figures/ours_small_comp.tex <==
\begin{figure*}
\includegraphics[width=\linewidth]{figures/Ours-small-comparison.pdf}
    \centering
    \caption{Comparison of ground truth images from the test set between ours-small compressed representation and 3DGS-7k.}
    \label{fig: ours-small}
    \vspace{-0.4cm}
\end{figure*}

==> display_figures/qbits.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/qbits_comparison.pdf}
    \caption{Comparison of performance at different bit-depths where opacity (o), scale (s), rotation (r), xyz position (x).}
    \label{fig:quant-comp}
\end{figure}

==> tables/quantization_level_comp.tex <==
\begin{table*}
    \caption{Comparison of the effect of different quantization bit levels on the Playroom and DrJohnson scenes from the Deep Blending dataset.}
    \label{tab: quant-comp}
    \centering
    \scalebox{0.9}{
    \begin{tabular}{ccccc|ccc|ccc}
    \toprule
          \multicolumn{5}{c}{Quantization Bit Level}  & \multicolumn{3}{c}{Play Room} & \multicolumn{3}{c}{Dr Johnson} \\
   SH-Features & Opacity & XYZ & Rotation & Scaling & SSIM$^\uparrow$ & PSNR$^\uparrow$ & LPIPS$^\downarrow$  &SSIM$^\uparrow$ & PSNR$^\uparrow$ & LPIPS$^\downarrow$ \\
    \midrule

8 & 16 & 16 & 16 & 16 & 0.855 & 27.820 & 0.316 & 0.539 & 10.624 & 0.768 \\
8 & 24 & 16 & 16 & 16 & 0.854 & 27.787 & 0.317 & 0.827 & 26.924 & 0.343 \\
8 & 24 & 24 & 16 & 16 & 0.893 & 29.473 & 0.256 & 0.891 & 29.042 & 0.254 \\
8 & 24 & 24 & 8 & 8 & 0.879 & 28.051 & 0.278 & 0.880 & 28.362 & 0.280 \\

    \bottomrule
    \end{tabular}
    }
\end{table*}
